Physics-Driven Learning of Wasserstein GAN for Density Reconstruction in Dynamic Tomography

Object density reconstruction from projections containing scattered radiation and noise is of critical importance in many applications. Existing scatter correction and density reconstruction methods may not provide the high accuracy needed in many applications and can break down in the presence of unmodeled or anomalous scatter and other experimental artifacts. Incorporating machine-learned models could prove beneficial for accurate density reconstruction particularly in dynamic imaging, where the time-evolution of the density fields could be captured by partial differential equations or by learning from hydrodynamics simulations. In this work, we demonstrate the ability of learned deep neural networks to perform artifact removal in noisy density reconstructions, where the noise is imperfectly characterized. We use a Wasserstein generative adversarial network (WGAN), where the generator serves as a denoiser that removes artifacts in densities obtained from traditional reconstruction algorithms. We train the networks from large density time-series datasets, with noise simulated according to parametric random distributions that may mimic noise in experiments. The WGAN is trained with noisy density frames as generator inputs, to match the generator outputs to the distribution of clean densities (time-series) from simulations. A supervised loss is also included in the training, which leads to improved density restoration performance. In addition, we employ physics-based constraints such as mass conservation during network training and application to further enable highly accurate density reconstructions. Our preliminary numerical results show that the models trained in our frameworks can remove significant portions of unknown noise in density time-series data.

==> writeup/header.tex <==
\usepackage{float}
\usepackage{bm}
% \usepackage{ulem}
\usepackage{extarrows}
% \usepackage{enumitem}
\usepackage{comment}
\usepackage{amsthm,amsmath,amsfonts}
\usepackage{booktabs}
% \usepackage[colorlinks=true]{hyperref} % preloaded in els article
% \usepackage[noend]{algorithmic}
% \usepackage[algo2e,ruled,linesnumbered]{algorithm2e}
% This is a bit nicer:
% \usepackage{algorithm,algpseudocode} % algorithmicx package

\usepackage{cleveref}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}

% \usepackage{natbib}
\usepackage{graphicx}
\usepackage{bbm}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\dis}{\displaystyle}
\newcommand{\E}{\mathbb{E}\,}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}
\renewcommand{\d}{\mathrm{d}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\tr}{\mathrm{Tr}}
% \newcommand{\Xtensor}{\mathcal{X}}
% \newcommand{\Ytensor}{\mathcal{Y}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}

% \newcommand{\argmin}[1]{\underset{#1}{\mathrm{argmin} \, }}
\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
   \node[shape=circle,draw,inner sep=1pt] (char) {\footnotesize #1};}}
   
\newcommand{\autocorr}{R} % single tau
% \newcommand{\Autocorr}{\mathbf{R}} % all tau
\newcommand{\Autocorr}{\mathbf{R}} % all tau
% \newcommand{\transpose}{\intercal} % or ... % SRB, this isn't working well
\newcommand{\transpose}{\top}
\newcommand{\trans}{\transpose}
\newcommand{\covmat}{\boldsymbol{\Sigma}}

==> writeup/introduction.tex <==
%Object density reconstruction from projections is of critical importance in national security, healthcare, and other applications. A key challenge to accurate density reconstruction is the presence of experimental artifacts in the measurements including scattered radiation and noise. Such artifacts pose challenges for modeling and correction.

The reconstruction of a density object from  line integrated radiographic projections, has a long history dating back to Radon~\cite{radon1917}.  Accordingly, in many scientific applications arising in material science, shock physics, inertial confinement fusion, and in nuclear security applications including stockpile stewardship a sequence of radiographic images are acquired and utilized in an attempt to elucidate the physics models and their associated parameters. However,  experimental dynamic radiographs  are complicated by the noisy and complex multi-scale and multi-physics environment. These complexities give rise to uncertainties in the density reconstructions from the inability to exactly represent various aspects of the radiographic measurement system, such as scatter, beam spot movement, beam-target interactions, beam dynamics repeatability, and aspects of the image formation process.
Modern approaches  to solving the radiographic inversion problem, and poly-energetic radiographic systems, with a complex non-linear/non-convex forward model generally employ iterative reconstruction techniques.  Mathematically we may express this problem as:
\begin{equation}
\hat{x} = \mathrm{arg} \min_x F(x) + \sum_i \alpha_i R_i(x)
\label{eq:opt_recon}
\end{equation}
where $F(x)$ is the data fidelity term capturing the forward model of the imaging process and the statistical models of measurements and noise, and the $R_i(x)$ are regularizer models for the desired image.  The scalar parameters $\alpha_i$ control the relative strength of the respective regularizers.  

The determination of the correct density distribution from \eqref{eq:opt_recon} is contingent not only upon formulating a proper physics-based forward model, but also imposing appropriate regularization and effective   schemes to solve the optimization problem. 

Figure \ref{fig:Forward}  depicts the objective of the forward modeling approach.


\begin{figure}[!h]
  \centering
  \includegraphics[width=0.7\textwidth]{figures/Forward_Model.png}
  \caption{Forward modeling approach to radiographic reconstruction}
  \label{fig:Forward}
\end{figure}

The application of the forward modeling approach to a French Test Object fielded at the Los Alamos Dual Axis Radiographic Hydrodynamic Test Facility (DARHT), Figure \ref{fig:FTO}, has enabled density reconstructions to be obtained.  The density errors using a radiographic forward model are depicted in Figure \ref{fig:FTO_errors}. 
\begin{figure}[!h]
    \centering
    \begin{subfigure}[b]{.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/LOS.png}
        \label{fig:LOS}
        \caption{A schematic of the DARHT radiographic scene.}
    \end{subfigure}%
    \begin{subfigure}[b]{.35\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/FTO_radiograph_MCNP_annotated.pdf}
        \label{fig:FTO_annotated}
        \caption{An FTO simulated radiograph.}
    \end{subfigure}
   \caption{The French Test Object (FTO) fielded at DARHT and a simulated radiograph with key features identified.}
  \label{fig:FTO}
\end{figure}
\begin{figure}[!h]
    \centering
   \includegraphics[width=.7\textwidth]{figures/FTO_BIEErrors.png}
   \caption{Density Errors of the French Test Object using a Forward Model.}
  \label{fig:FTO_errors}
\end{figure}

  While the density reconstructions obtained using the traditional radiographic iterative reconstruction approach would appear to be reasonable, they are not in general sufficient to elucidate physics of many of the fundamental issues e.g. Equation of State Modeling and constitutive properties of the materials. Thus, incorporating learned models of the underlying dynamics is of much importance for accurate density reconstruction. This may be particularly useful in dynamic imaging, where the time-evolution of the underlying density fields could be captured by learning from large hydrodynamics simulations, wherein various physics-based properties could also be incorporated during learning.

In this work, we demonstrate the ability of a learned generative adversarial network (GAN) for  artifact removal in noisy density reconstructions, where the noise is imperfectly characterized. The generator in the GAN serves as a denoiser that removes artifacts in densities obtained from traditional scatter correction and density reconstruction algorithms. We train the GAN from large density time-series datasets obtained from hydrodynamic simulations, with noise simulated according to parametric random distributions that may mimic noise in experiments. Essentially, the GAN is trained with noisy density frames as generator inputs, to match the generator output distribution to the distribution of clean densities (time-series) from the hydrodynamic simulations. We studied the Wasserstein-GAN in our experiments. Primitive numerical results show that the denoisers trained in the GAN frameworks are capable of removing significant portions of existing unknown noise in density time-series.

In addition, we have found that the use of physics-based constraints during network training and application allows for more accurate density reconstructions that are more consistent with the underlying hydrodynamics. In particular, we leveraged mass conservation over time as prior knowledge by incorporating an additional penalty term during both training and testing. Such a prior improved the quality of density reconstructions in our framework. Primitive experimental results are presented in the following figures. 



 
